Computing All Restricted Skyline Probabilities on Uncertain Datasets

Restricted skyline (rskyline) query is widely used in multi-criteria decision making. It generalizes the skyline query by additionally considering a set of personalized scoring functions F. Since uncertainty is inherent in datasets for multi-criteria decision making, we study rskyline queries on uncertain datasets from both complexity and algorithm perspective. We formalize the problem of computing rskyline probabilities of all data items and show that no algorithm can solve this problem in truly subquadratic-time, unless the orthogonal vectors conjecture fails. Considering that linear scoring functions are widely used in practical applications, we propose two efficient algorithms for the case where $\calF$ is a set of linear scoring functions whose weights are described by linear constraints, one with near-optimal time complexity and the other with better expected time complexity. For special linear constraints involving a series of weight ratios, we further devise an algorithm with sublinear query time and polynomial preprocessing time. Extensive experiments demonstrate the effectiveness, efficiency, scalability, and usefulness of our proposed algorithms.

==> introduction.tex <==
\section{Introduction}\label{sec:introduction}
%1. start with uncertian data, then why skyline and top-k is not work
%2. start with rskyline, then uncertainty is inherent in real dataset
The top-$k$ query and the skyline query are widely used in \textit{multi-criteria decision making}~\cite{koksalan2011multiple}.
Given a dataset, the former reports $k$ highest-scoring tuples according to a user-specified scoring function, while the latter outputs a set of all non-dominated tuples, where a tuple $t$ dominates another tuple $s$ if $t$ is no worse than $s$ in all dimensions and better than $s$ in at least one dimension.
However, it has been recognized that focusing on either of these two queries individually has some unavoidable drawbacks.
For example, the top-$k$ results depend heavily on the user-specified scoring function and thus only provides a narrow view of the dataset.
Meanwhile, the requirement that an exact scoring function is known in advance is also hardly realistic in practice.
As for the skyline, although it includes all possible tuples of interest, its size may be too large for users to come up to a final decision.

With the aim of gathering the strengths of these two queries while avoiding their drawbacks,  Ciaccia and Martinenghi~\cite{DBLP:journals/pvldb/CiacciaM17} recently introduced a notion of restricted skyline (rskyline).
By considering a set of user-specified scoring functions $\calF$, they defined that a tuple $t$ $\calF$-dominates another tuple $s$ if $t$ scores better than $s$ under any function $f \in \calF$, and the rskyline query is to retrieve the set of all non-$\calF$-dominated tuples.
Note that the rskyline query is more general than the top-$k$ query because it does not require users to specify exact weight values with absolute accuracy, but rather an approximate description of their preferences.
Meanwhile, it is experimentally verified~\cite{DBLP:journals/pvldb/CiacciaM17} that the rskyline query significantly reduces the size of the skyline and provides an overview of all potentially interesting tuples with respect to functions in $\calF$.

However, it has been observed that data uncertainty is inherent in multi-criteria decision making from various causes such as, limitations of measuring equipment, data randomness and incompleteness, outdated sources, and so on~\cite{DBLP:journals/fcsc/LiWLG20}.
Although a considerable amount of research has been dedicated to answering the top-$k$ query~\cite{DBLP:conf/icde/SolimanIC07, DBLP:conf/icde/YiLKS08, DBLP:conf/icde/HuaPZL08, DBLP:journals/dpd/WangSY16} and the skyline query~\cite{DBLP:conf/vldb/PeiJLY07, DBLP:conf/pods/AtallahQ09, DBLP:journals/tods/AtallahQY11, DBLP:journals/mst/AfshaniAALP13, DBLP:journals/tkde/KimIP12, DBLP:journals/tjs/Gavagsaz21, DBLP:conf/icdcs/ZhangWWH19, DBLP:journals/is/ZhangZLJP11} on uncertain datasets, how to conduct rskyline analysis on uncertain datasets remains an open problem at large.
We first describe some application scenarios as follows:

\noindent{\it E-commerce Scenario:}
Data uncertainty is often found in e-comme-rce.
For example, vehicles in a used car platform (\eg, www.motors.ebay.com) may not always be available to the users for sure during the decision making process of a potential buyer.
Thus, each car actually has a probability of being available to users.
Suppose the two criteria in deciding which car a user wants are \textsf{Price} and \textsf{Mileage}, we can translate the preference for cheaper cars into a constraint on weights of a scoring function, \eg, focusing on the family $\calF = \{\omega_P \textsf{Price} + \omega_M \textsf{Mileage} \mid \omega_P \ge \omega_M \}$.
Conducting rskyline analysis on the vehicles dataset will quantify how likely a car is to be excellent with respect to some scoring function in $\calF$.

\noindent{\it Player Selection Scenario:}
Often times we cannot precisely specify and interpret the scoring function used to measure the performance of a player.
It is much easier for us to provide a relative importance of the attributes, \eg, \textsf{Points} is as least as important as \textsf{Assists}.
Input with a family of scoring functions $\calF$ satisfying such constraint, rskyline analysis on the technical statistics data of players helps to identify excellent players~\cite{DBLP:journals/pvldb/CiacciaM17}.
However, the performance data may vary substantially player by player and game by game.
And uncertainty is inherent due to many factors such as fluctuations of players’ conditions, the locations of the games, and the support from audience.
Modeling the game-by-game performance data as an uncertain dataset, then conducting probabilistic rskyline analysis will identify the players with high probability of excelling under some functions in $\calF$

\eat{
\noindent\underline{College Application Scenario:}
Assume a high school graduate receives a set of college admission offers. Although the graduate cannot set an exact attribute weight ratio for the two attributes, he specifies that major ranking is as least as important as university ranking.
However, rankings provided by different agencies are different.
Thus, we can treat the college as an uncertain object and the rankings as its instances.
Now, the probability can be the confidence of the ranking provided by each agency.
In such case, an offer with high rskyline probability means that this college is the top-1 choice for the graduate with some preference meeting his demands.
}
Motivated by these applications, we revisit the rskyline query on uncertain datasets in this paper.
We follow the uncertain model introduced in~\cite{DBLP:conf/pods/AtallahQ09}, in which the probability distribution of an object is represented by a weighted set of tuples called instances.
Given a set of scoring functions $\calF$, we define the probability of an instance being in the rskyline, called rskyline probability, as the probability that none of instances from other objects that $\calF$-dominates it occurs in the dataset.
And we investigate the problem of computing rskyline probabilities of all instances from both complexity and algorithm perspective.

For the problem complexity, we establish a fine-grained reduction from the Orthogonal Vectors problem to the problem of computing rskyline probabilities of all instances and prove that there is no truly subquadratic-time algorithm for all rskyline probabilities (ARSP) computation unless the Orthogonal Vectors conjecture fails.
It is noticed that the conditional lower bound also holds for all skyline probability (ASP) computation.
Note that although several efficient algorithms for this problem have been proposed in previous work~\cite{DBLP:conf/pods/AtallahQ09, DBLP:journals/tods/AtallahQY11, DBLP:journals/tkde/KimIP12, DBLP:journals/mst/AfshaniAALP13}, none of them considered the lower bound for this problem.
In~\cite{DBLP:journals/tods/AtallahQY11}, Atallah~\etal only made a discussion about the potential optimality of their algorithm but did not provide a formal proof.
This conditional lower bound first formally proves that the algorithms proposed in~\cite{DBLP:conf/pods/AtallahQ09, DBLP:journals/tods/AtallahQY11, DBLP:journals/mst/AfshaniAALP13} are near-optimal.

%TODO:introduce challenges for algorithmic results
As for the algorithmic concern, we focus on a practically effective case where $\calF$ consists of linear scoring functions described by a set of linear constraints.
%In many applications, especially in databases containing numeric attributes, the scoring function used to model user preferences is expressed in the form of a linear combination of query attributes.
%And a practical way to specify the preference region of a user is starting with $\simplex^{d-1}$ and adds some constraints.
Exploiting the convexity of the preference region, we transforms the ARSP computation in the original space into the ASP computation in the score space defined by the vertices of the preference region.
This leads to an algorithm with near-optimal time complexity for ARSP computation compared to the proved conditional lower bound.
And we also optimize the implementation of the called algorithm, which further enhances its experimental performance.
It is noticed that a major drawback of the above algorithm is all instances need to be mapped into the score space each time.
We resolve this by designing effective pruning strategies and conducting the mapping in an incremental manner.
By integrating them into the branch-and-bound paradigm, we propose an algorithm with better expected time complexity.

For a special case where linear constraints are $d - 1$ ratio bound constraints, we establish a Turing reduction from the ARSP computation to the half-space range searching problem using the well-known point-hyperplane duality.
Based on the reduction, we propose an $O(2^dmn\log{n})$-time algorithm with a polynomial-time preprocessing, where $m$ and $n$ is the number of objects and instances, respectively.
Subsequently, we introduce a multi-level structure and a data-shifting strategy to further improve the time complexity to $O(2^{d-1}\log{n} + n)$, where the additional linear time is only required for reporting the final results.
This algorithm matters from the following two aspects.
First, it proves that the online rskyline probability query belongs to the pseudo-logarithmic-time complexity class $\mathrm{PsL}$~\cite{DBLP:journals/tcs/GaoLML20}, which can be further used to design efficient algorithms for other queries.
Second, although this algorithm is somewhat inherently theoretical, experimental results shows that its extension for this special rskyline query on certain datasets outperforms the state-of-the-art method proposed in~\cite{DBLP:conf/icde/Liu0ZP021}.

To the best of our knowledge, this paper is the first work conducting rskyline analysis on uncertain datasets.
The main contributions of this paper are summarized as follows.
\begin{enumerate}[$\bullet$]
	\item We formalize the problem of computing all rskyline probabilities of all instances and prove a conditional lower bound that there is no algorithm can solve this problem in $O(n^{2-\delta})$ time for any $\delta > 0$, unless the Orthogonal Vectors conjecture fails.
	\item When the preference region is described by a set of linear constraints, for ARSP computation, we propose an algorithm with near-optimal time complexity $O(n^{2 - 1/d'})$, where $d'$ is the number of vertices of the preference region, and an algorithm with time complexity $O(mn\log{n})$ in expectation.
	\item When the preference region is specified by $d-1$ ratio bound constraints, we propose a $O(2^{d-1}\log{n} + n)$-time algorithm with a polynomial-time preprocessing for ARSP computation, and a $O(2^{d-1}\log{n})$-time algorithm with a polynomial-time preprocessing for online rskyline probability query.
	\item We conduct extensive experiments over real and synthetic datasets to demonstrate the effectiveness of ARSP computation and the efficiency and scalability of the proposed algorithms.
	%	Moreover, the extension of the sublinear-time algorithm also outperforms the state-of-the-art method for the restricted skyline query on certain datasets.
\end{enumerate}

The reminder of this paper is organized as follows.
We review the related work in Section~\ref{sec:relatedwork}.
We formally define the problem studied in this paper and study its conditional lower bound in Section~\ref{sec:preliminary}.
Then, we propose two efficient algorithms for ARSP computation in Section~\ref{sec:rskyprobalg}, and design an algorithm with sublinear query time and polynomial preprocessing time for ratio bound constraints in Section~\ref{sec:eclprobalg}.
We report the experimental results in Section~\ref{sec:experiments}.
Finally, we conclude the paper in Section~\ref{sec:conclusions}.

==> response.tex <==
\noindent{\bf \large REVISION LETTER}
%\BlankLine\BlankLine
%\noindent Dear reviewers,
%\BlankLine\BlankLine
%\noindent 

Thank you very much for your valuable feedback.
%\BlankLine\BlankLine
%\noindent 
We appreciate the depth of your reviews and the work you spent towards our paper.
We carefully implemented your suggestions and high-lighted the changes in \textcolor{blue}{blue} in the revised paper. % and think that based on the reviews, we were able to substantially improve the paper.
%\BlankLine\BlankLine
%\noindent
%We made extensive changes with regard to the motivation of studied problem, reasonableness of the model, improvements of the experimental study, presentation of the paper, and revised discussions.
%In the revised paper, the changes are high-lighted in \textcolor{blue}{blue}.
%For figures that were added or changed, we marked the captions in blue.
The major changes of our paper are summarized as follows.

(1) We updated the real-life applications in section I.

(2) We rewrote the sixth paragraph of section I to emphasized the difference between our work and the existing work.
And we also discussed detailed differences in section II.

(3) We redefined the rskyline probability based on possible world semantics~\cite{DBLP:conf/sigmod/AbiteboulKG87} in section III.B, which equals to previous one, and redesigned example 1 and figure 1 to explain it.

(4) We removed summary of notations due to lack of space.

(5) We formally defined linear constraints with matrix in-equality in the first paragraph of section IV.

(6) We added an enumeration-based based baseline.

(7) We redesigned example 3, 4, and figure 3 to provided more intuitive explanation of the proposed algorithm.

(8) We improved the description of multi-level strategy.

(9) We added two real datasets IIP~\cite{DBLP:journals/vldb/JinYCYL10} and CAR~\cite{DBLP:journals/tkde/LiuYYL13}. %which were also used in previous work on query processing over uncertain datasets, .
We also expanded the NBA dataset in terms of both data cardinality and data dimensionality.
Now, it contains 354,698 game records of 1,878 players with 8 attributes.
%Now, it contains 668,003 game records of 3,218 players with 8 attributes.
%We extracted 994,031 game records of 3,502 players with 7 attributes from~\url{https://www.nba.com/stats/}.
Code for generating these datasets can found at~\cite{github}.
Details of these three datasets and methods to generate existence probabilities for records in these datasets can be found in the first paragraph of section VI.A.
%We added two real datasets IIP and CAR, and expanded the NBA dataset in terms of both data cardinality and data dimensionality.
%We described the methods to generate existence probabilities following the descriptions of datasets.

(10) We removed the table for parameter settings and introduced them at the beginning of section VI.C. 
We also added references for parameter settings and involved constraints.

(11) We re-conducted the experiments for verifying the effectiveness of ARSP on NBA in section IV.B.
We compared ARSP and the aggregated rskyline by selecting four representative players.
And all statements were derived based on their score distributions (see figure~\ref{fig:score}).
%We re-conducted the experiments for verifying the effectiveness of ARSP and added figure 4 to show score distributions of four representative objects in section VI.B.

(12) We added experiments to evaluate the effect of each parameter on the number of instances with none-zero rskyline probabilities.
The results were plotted at the second y-axis of each experimental figure in section IV.C.
%We added experiments about the number of instances with non-zero rskyline probabilities in section VI.C.

(13) We reported the performance of proposed algorithms on real and correlated synthetic datasets in section VI.C.

(14) We replotted experimental results of section VI.C.

The following is our detailed responses to your comments.

%\BlankLine\BlankLine
%\noindent The authors
%\BlankLine\BlankLine
\noindent{\bf Detailed Comments to Meta Review}

%\begin{mybox}[]{Meta Review - R1}
%	Improve the motivation for the studied problem.
%\end{mybox}
{\bf R1.}
We improved the motivation for the studied problem from the following two aspects.
%add application

(1) We provided two more real-life scenarios that the studied problem can be applied in the revised introduction.
Since Reviewer 4 O1 pointed out that booking probabilistic hotels is not common in practice as users usually select a specific hotel, instead of a region, we rewrote the e-commerce scenario with car rental services provided on Hotwire (\url{www.hotwire.com/car-rentals/}).
In this case, the uncertain data comes from the sale strategy and $\calF$ describes a user's imprecise preference for cars' attributes. 
We also introduced the application of our problem to stock market prediction services.
The existence probability of data reflects the confidence of the prediction and $\calF$ describes the user's rough preference for selecting stocks.
In addition, our problem can also be used in sensor datasets (\eg, IIP in our experiments).
The uncertainty comes from the limitations of equipment, and $\calF$ contains the scoring functions for evaluating the status of an iceberg.
Also, in job hunting scenario described in~\cite{DBLP:conf/pods/AtallahQ09}, the probability shows the likelihood of a job being offered to the applicant.
And $\calF$ to our problem can be used to characterize the applicant's requirement that if the job-security decrease by 1, then the salary must increase by 1000 ($\calF = \{\omega_1 Salary + \omega_2 Security \mid \omega_1 \ge 1000 \omega_2\}$).

%distinguish between previous work
(2) We emphasized the difference between our work and the existing work.
Previous researches on uncertain datasets performed different tasks, such as skyline queries~\cite{DBLP:conf/vldb/PeiJLY07, DBLP:journals/is/ZhangZLJP11, DBLP:journals/ijon/YangLZMG18, DBLP:journals/isci/YongLKH14}, top-$k$ queries~\cite{DBLP:conf/icde/HuaPZL08, DBLP:conf/icde/SolimanIC07, DBLP:journals/dpd/WangSY16, DBLP:conf/icde/YiLKS08, DBLP:conf/sigmod/GeZM09}, \etc
They only considered uncertainty in datasets but not in user preferences.
However, as stated in~\cite{DBLP:journals/pvldb/MouratidisT18, DBLP:conf/sigmod/MouratidisL021}, determining a precise scoring function for a user, which is required for top-$k$ queries, is unrealistic and skyline queries lack personalization.
%However, it is not reasonable to expect a user to precisely determine the scoring function like top-$k$ queries, even though he/she may roughly know what to look for~\cite{DBLP:journals/pvldb/MouratidisT18, DBLP:conf/sigmod/MouratidisL021}.
%Meanwhile, skyline queries lack of personalization.
%The input set $\calF$ describes the fuzzy scoring function of a single user o
Our problem overcomes this by including all possible scoring functions of the user in $\calF$, which can be efficiently mined by learning techniques like~\cite{DBLP:journals/pvldb/QianGJ15}.
And works involving uncertain preferences~\cite{DBLP:journals/pvldb/CiacciaM17, DBLP:journals/pvldb/MouratidisT18, DBLP:conf/icde/Liu0ZP021, DBLP:conf/sigmod/MouratidisL021} only consider datasets without uncertainty.
Our work extend the $\calF$-dominance-based operators~\cite{DBLP:journals/pvldb/CiacciaM17} to uncertain datasets.

%\begin{mybox}[]{Meta Review - R2}
%	Justify the independence assumption and explain the existential probability model.
%\end{mybox}

{\bf R2.}
%The model used in 
It was pointed out the independence assumption may be violated in player selection scenario.
However, the assumption do hold in a lot of applications.
In e-commerce scenario, when a customer rents a compact SUV from Hotwire, he may be offered a Ford Eco Sport or similar with the predetermined probability.
This will not affect the probability of offering any car to him when he rents a mid-size sedan.
Thus, two objects (probabilistic cars here) are independent.
In prediction service, the learning algorithm's output for two stocks is independent.
In sensor dataset, the confidence of records collected by a sensor only depends on its own device accuracy.
Moreover, the same assumption can be found in almost all work on uncertain skyline queries~\cite{DBLP:conf/vldb/PeiJLY07, DBLP:journals/is/ZhangZLJP11, DBLP:journals/ijon/YangLZMG18, DBLP:journals/isci/YongLKH14, DBLP:conf/pods/AtallahQ09, DBLP:journals/tods/AtallahQY11, DBLP:journals/mst/AfshaniAALP13, DBLP:journals/tkde/KimIP12, DBLP:journals/tkde/LiuYYL13}.
This also explains the meaning of existence probability.
In probabilistic car renting, it means the likelihood that a user can get Ford Eco Sport if he rents a compact SUV.
And in prediction service and sensor dataset, it characterize the confidence of the data.

%\begin{mybox}[]{Meta Review - R3}
%	Clarify technical discussions and the costs/benefits of Algorithms 1 \& 2.
%\end{mybox}

{\bf R3.}
The reason why the KD-tree is constructed on-the-ﬂy in algorithm 1, while all instances are organized into an R-tree in advance in algorithm 2 is as follows.
If the uncertain dataset is static, given any input $\calF$, algorithm 2 can process $\calF$ by performing the best-first traverse on the same R-tree.
Different $\calF$ only affect the min-heap used in Algorithm 2 but do not affect the R-tree structure on $I$.
And when the dataset is updated, it is also efficient to update the R-tree.
However, given an input $\calF$, algorithm 1 first needs to compute $S_{_V}(t)$ for each $t \in I$, where $V$ is the set of vertices of the preference region in $\calF$, and then constructs a KD-tree on $I' = \{S_{_V}(t) \mid t \in I\}$.
Different $\calF$ result in different sets $I'$, thus also different KD-trees.
Therefore, we do not consider the construction time of the R-tree on $I$ in the efficiency evaluation of algorithm 2.
This is reasonable since the construction is a one-time cost for all subsequent input $\calF$.
The same assumption can also be found in previous related work~\cite{DBLP:journals/pvldb/MouratidisT18}.
And we consider the construction time of the KD-tree in the efficiency evaluation of algorithm 1 and the construction time of $m$ aggregated R-trees in the efficiency evaluation of algorithm 2, since they all need to be built from scratch for different $\calF$.
We clarified this in the first paragraph of section IV.C.

%\begin{mybox}[]{Meta Review - R4}
%	Enhance the experiments as per the review comments.
%\end{mybox}

{\bf R4.}
We enhanced the experiments according to the comments of each reviewer.
Details can be found at (6), (9), (11), (12), (13), and, (14) of the change summary.

\eat{
The major changes are summarized as follows.

%real dataset
(1) We added two real datasets IIP~\cite{DBLP:journals/vldb/JinYCYL10} and CAR~\cite{DBLP:journals/tkde/LiuYYL13}. %which were also used in previous work on query processing over uncertain datasets, .
We also expanded NBA dataset in terms of both data cardinality and data dimensionality.
Now, it contains 994,031 game records of 3,502 players with 7 attributes.
%We extracted 994,031 game records of 3,502 players with 7 attributes from~\url{https://www.nba.com/stats/}.
Code for generating these datasets can found at~\cite{github}.
Details of these three datasets and methods to generate existence probabilities for records in these datasets can be found in the first paragraph of section VI.A.

%effectiveness of ARSP
(2) We re-conducted the experiments for verifying the effectiveness of ARSP on NBA.
We compared ARSP and the aggregated rskyline by selecting four representative players and displaying their score distributions with boxplots (Fig.~\ref{fig:score}).

%analyze of size of ARSP
(3) We evaluated the effect of each parameter on the number of instances with none-zero rskyline probabilities (the second y-axis of each experimental figure).

(4) Some minor modifications.
We added an enumeration-based baseline algorithm and added references for parameter settings and constraints generation methods.
We included the experimental results on real and correlated synthetic datasets.
We also replotted all experimental figures.
}
%\clearpage

%\BlankLine\BlankLine
\noindent{\bf Detailed Comments to Reviewer 3}

\eat{
\begin{mybox}[]{Review 3 - O1}
	It is not well motivated why probabilistic rskyline query is essential. E-commerce scenario and player selection scenario are provided by the authors, but it seems they can be answered by probabilistic top-k skyline query, which is well studied in the past few years.\newline
	[Efficiently Answering Probabilistic Threshold Top-k Queries on Uncertain Data. ICDE 2008]\newline
	[Preference-Based Top-k Representative Skyline Queries on Uncertain Databases. PAKDD 2015]\newline
	[Exact processing of uncertain top-k queries in multi-criteria settings. PVLDB 2018]\newline
	[Top k probabilistic skyline queries on uncertain data. Neurocomputing 2018]
\end{mybox}
}

{\bf O1.}
As stated in the response to Meta Review-R1, our problem considered uncertainty not only in datasets, but also in users' preferences.
%Finding objects with top-$k$ skyline probabilities does not satisfy the preference specified by $\calF$.
Unlike probabilistic top-$k$ skyline queries (\eg,~\cite{DBLP:journals/ijon/YangLZMG18}), the additional input $\calF$ describes a user's preference, which can contain any number of scoring functions. 
This is also different from uncertain the top-$k$ query (\eg,~\cite{DBLP:conf/icde/HuaPZL08}) since it requires that only one exact scoring function can be provided.
Moreover, since the rskyline result is always a subset of the skyline result, given a set of scoring functions $\calF$, a skyline object may be $\calF$-dominated by other objects.
Therefore, an object with high skyline probabilities may have low rskyline probabilities, making it less attractive under $\calF$.
Work like~\cite{DBLP:journals/pvldb/MouratidisT18} studied queries with uncertain preference on certain datasets.
As for \cite{DBLP:conf/pakdd/NguyenC15}, it considered dominance-based queries with user-specified priority of dimensions on uncertain datasets.
Whereas, $\calF$ to our problem can describe more kinds of the user's scoring functions.

\eat{
\begin{mybox}[]{Review 3 - O2}
	There are existing papers that generalize both skyline and ranking queries on uncertain datasets, which is exactly the target of probabilistic rskyline query. The authors should clearly point out the research gap between probabilistic rskyline query and probabilistic skyline ranking queries.\newline
	[Ranking uncertain sky: The probabilistic top-k skyline operator. Information Systems 2011]\newline
	[Skyline ranking for uncertain databases. Information Sciences 2014]
\end{mybox}
}

{\bf O2.}
Our problem is completely different from theirs.
These works aim to retrieve $k$ uncertain objects with the highest skyline probabilities. 
We aim to compute all uncertain objects' rskyline probabilities.
The rskyline probabilities can better serve the specific preferences of individual users, i.e., given different input $\calF$, the rskyline probabilities of uncertain objects are different.
However, the skyline probability of an uncertain object also remains the same for any user.

\eat{
\begin{mybox}[]{Review 3 - O3}
	The authors list much related work in Section 2, but the research gap is not well described, especially for the key references.
\end{mybox}
}

{\bf O3.}
In the revised version, we pointed out the differences between our problem and existing ones in section I and II.
%We also added descriptions of key references as your command.

\eat{
\begin{mybox}[]{Review 3 - O4}
	It is suggested to add a naive baseline that simply enumerates the instances of the uncertain objects and summarizes the possible worlds where the target object becomes rskyline.
\end{mybox}
}

{\bf O4.}
%Yes, we did.
The algorithm is introduced in the first paragraph of section IV.A and experimental studies can be found in section VI.
However, due to its exponential time complexity, the baseline cannot finish within the limited time even under the least time-consuming parameter settings.


\eat{
\begin{mybox}[]{Review 3 - O5}
	The authors claim that aggregated rskyline loses important distribution information and the result may not be meaningful.
	However, from the current results in Table 3, it is hard to say ARSP is more comprehensive than aggregated rskyline.
	More experiment results need to be provided to support the statement.
	Otherwise, it is hard to say the uncertain semantics are suitable for rskyline queries.
\end{mybox}
}

{\bf O5.}
%In the revised experiments, we used boxplots to represent players' score distributions and conducted a more detailed analysis of these two results with four concrete players.
Please refer to (11) of the change summary.

\eat{
\begin{mybox}[]{Review 3 - O6}
	In the introduction part, it is suggested to provide more meaningful applications to illustrate real-world rskyline queries with inherent uncertainty.
	For the scenario of player selection, the authors point out that the uncertainty comes from fluctuations of players' conditions, the locations of the games, the support from audience, etc. However, these factors may violate the independence assumption, and its existence probability is still unclear.
\end{mybox}
}

{\bf O6.}
%Yes, we provided two more real-life applications of our problem in the revised introduction.
%A brief description of more applications can be found in the response to Meta Review-R1.
%And we justified the independence assumption and explained the meaning of existence probability in the response to Meta Review-R2.
Please refer to the reply to Meta Review-R1 and R2.

\eat{
\begin{mybox}[]{Review 3 - O7}
	In the methodology part, KD-tree is constructed on the ﬂy in Algorithm 1, while all instances are organized into R-tree in advance in Algorithm 2.
	Is the tree construction time involved in the efficiency evaluation?
	How to balance the construction cost and efficiency benefits?
\end{mybox}
}

{\bf O7.}
%Sorry for our unclear description.
Please see the response to Meta Review-R3 for details. 

\eat{
\begin{mybox}[]{Review 3 - O8}
	The real dataset is rather small in player number and attribute number, and unclear how to generate the existence probabilities.
\end{mybox}
}

{\bf O8.}
%We expanded the NBA dataset in terms of both data cardinality and attribute number and explained how to generate the existence probabilities.
This is a helpful comment as the original NBA dataset is too small to verify the performance of proposed algorithms.
As stated in (9) of the change summary, we not only expanded the NBA dataset in terms of data cardinality and attributes number, but also added two real datasets.
%See the response to Meta Review-R4 for details.


\eat{
\begin{mybox}[]{Review 3 - O9}
	It is suggested to add references or supports for the parameter settings and constraints, e.g., interactive constraints.
\end{mybox}
}

{\bf O9.}
Parameter settings for synthetic datasets followed the previous work on skyline queries processing over uncertain datasets~\cite{DBLP:conf/vldb/PeiJLY07, DBLP:journals/tkde/KimIP12}.
Since they did not verify the effects of $cnt$, $l$, and $\phi$, we only set default values as they did, and then set ranges ourselves.
%In addition to $m$ and $d$ considered in~\cite{DBLP:conf/vldb/PeiJLY07, DBLP:journals/tkde/KimIP12}, we also verify the effects of $cnt$, $l$, and $\phi$.
As for methods to generate constraints, we involved the WR method as specifying rankings on attributes is one of the most common ways to express preference~\cite{DBLP:journals/cor/EumPK01} and WR was also considered in the first work for rskyline queries~\cite{DBLP:journals/pvldb/CiacciaM17}.
Moreover, inspired by preference learning techniques like~\cite{DBLP:journals/pvldb/QianGJ15}, we considered the IM method.
In practice, it is easy and cheap to obtain a user's rough preferences by asking him/her to compare several pairs of options.
These references were all added in the revised paper.

%\clearpage

%\BlankLine\BlankLine
\noindent{\bf Detailed Comments to Reviewer 4}

\eat{
\begin{mybox}[]{Reviewer 4 - O1}
	The studied problem is not well motivated.
	\begin{itemize}
		\item[(1)] The authors need to provide more real-life scenarios that the studied problem can be applied.
		The provided case of uncertain hotel may not be a good one, since users usually select a specific hotel, instead of a region (meanwhile, it is hard to define this region).
		\item[(2)] In the fourth paragraph of Section 1, the authors mentioned that the calculated rskylines on aggregation points (over uncertain data) may be meaningless in their evaluation.
		Please briefly discuss the experimental results here.
	\end{itemize}
\end{mybox}
}

{\bf O1.}
(1) Please refer to the response to Meta Review-R1.

(2) In the sixth paragraph of Section I, we added a discussion about why the aggregated result may be meaningless and fails to provide comprehensive view on uncertain datasets.

\eat{
\begin{mybox}[]{Reviewer 4 - O2}
	The experiments can be improved.
	\begin{itemize}
		\item[(1)] It would be good if the authors can find and evaluate on more real-life datasets.
		\item[(2)] For the baseline, it would be good if the authors can compare their methods with some of the rskyline methods on certain datasets.
		If I understand correctly, the existing approaches can be slightly revised to solve the studied problem, with a low efficiency.
		\item[(3)] For the synthetic datasets, why do the authors ignore the correlated datasets?
		\item[(4)] The authors may consider release the number of rskylines (with probabilities greater than 0) on the tested datasets.
	\end{itemize}
\end{mybox}
}

{\bf O2.}
%We improved the experiments based on your comments.
(1) We involved three real datasets in the revised experiments.
See (9) of the change summary for details.

(2) Actually, the original baseline is an extension of rskyline algorithms on certain datasets proposed in~\cite{DBLP:journals/pvldb/CiacciaM17}.
We renamed it LOOP in the revised version and compared it with our proposed methods under all parameter configurations.
%Or put it on arxiv

(3) As correlated datasets are the least challenging when it comes to computing skyline or rskyline, we ignored them for lack of space.
% In the revised version, we included the results on correlated datasets.
% and placed other results in the full version of the paper~\cite{gao2023computing}.
%The results on correlated datasets can be found in the full version of our paper~\cite{gao2023computing}.
In the revised paper, we reported the results on correlated datasets in section IV.C.

(4) This advice is helpful.
We added experimental results about this number as stated in (12) of the change summary.
%We evaluated the effect of each parameter on the number of instances with non-zero rskyline probabilities.
%In the revised paper, we released the number of instances with none-zero rskyline probabilities in our experimental results (see the second y-axis of each parameter figure) and discussed the effects of each parameter on this number.
%The details can be found in the *** item of the response to Meta Review - R4.

\eat{
\begin{mybox}[]{Reviewer 4 - O3}
	Some technical discussions are not clear.
	\begin{itemize}
		\item[(1)] In the first paragraph of Section IV, the symbol $A$ is not defined.
		\item[(2)] In the last paragraph of Section IV, the symbol $n$ is not defined (shown in the complexity analysis of Algorithm 2).
	\end{itemize}
\end{mybox}
}

{\bf O3.} Thanks for careful reviewing.
We checked our paper to ensure that all symbols were used after formal definition.
%\clearpage

%\BlankLine\BlankLine
\noindent{\bf Detailed Comments to Reviewer 5}

\eat{
\begin{mybox}[]{Reviewer 5 - D1}
	In the experimental part of Chapter VI, the figures used for showing runtime are mostly depicted with solid black lines.
	The experimental display effect is not clear enough, it is recommended to use different colors and line shapes for different algorithms.
\end{mybox}
}
{\bf D1.}
Thanks for your advice.
We replotted all experimental figures following your comment.

\eat{
\begin{mybox}[]{Reviewer 5 - D2}
	In Sections C and D, the runtime is studied mostly with synthetic datasets.
	It will be better if more real datasets are used to demonstrate the algorithms’ efficiency.
	In the analysis and research of factors that affect runtime, it is recommended to add the result of the baseline for comparison.
\end{mybox}
}
{\bf D2.}
%In the revised version, we added two real datasets IIP and CAR in our experimental studies (see the response to Meta Review-R4 for details).
As stated in (9) of the change summary, we involved three real datasets in the revised experiments.
%Please refer to the response to Meta Review-R4 for details.
We also plotted the baseline results as a reference in every experimental figure.

\eat{
\begin{mybox}[]{Reviewer 5 - D3}
	The context of Example 3 is complex, but the descriptions in Figure 3 and Example 3 are relatively brief and do not provide a sufficiently intuitive description of the process.
	It would be better if the analysis and explanation of the examples were more detailed and clear.
\end{mybox}
}

{\bf D3 D5.}
We redesigned Example 3 and 4 to provide more intuitive explanation of the proposed algorithm.
In Example 3, we used an uncertain dataset to illustration the reduction.
We explained how to partition the data space with an instance and plotted the hyperplane used to find all instances that $\calF$-dominate this instance in each region.
In Example 4, we continued with one resulted region in Example 4 and showed the information kept for each face in that region.
Then, we explained how to use this information to compute the rskyline probability of this instance. 

\eat{
\begin{mybox}[]{Reviewer 5 - D4}
	The description of Multi-level strategy could be improved.
	For example, it would be better to declare the correspondence between the structure level and the point location query.
	Then, in the query processing stage, it will be more clear which dual point is being located on current level and how to get next level of the structure.
\end{mybox}
}

{\bf D4.}
We rewrote the description following your suggestion.

\eat{
\begin{mybox}[]{Reviewer 5 - D5}
	Examples for Chapter V should be redesigned to provide a more intuitive explanation of the maintained information and how to process the query.
\end{mybox}
}


\eat{
\begin{mybox}[]{Reviewer 5 - D6}
	The font in Figure 3 and Figure 8 (a) is too small to read.
\end{mybox}
}

{\bf D6.}
Sorry for our mistake.
We replotted these two figures and checked the other figures to ensure their readability.

\eat{
\begin{mybox}[]{Reviewer 5 - D7}
	As the major theoretical contribution, it should be better to involve a proof sketch of Theorem 1 in the paper.
\end{mybox}
}

{\bf D7.}
For lack of space, we finally putted them on arxiv~\cite{gao2023computing}.

\eat{
\begin{mybox}[]{Reviewer 5 - D8}
	It would be better to claim why the proposed sublinear-time algorithm does not work with general linear constraints.
\end{mybox}
}

{\bf D8.}
%Given general linear constraints $A \times \omega \le b$, we can also establish a similar reduction to the half-space reporting problem by computing the set of vertices $V$ of $\Omega = \{\omega \in \simplex^{d-1} \mid A \times \omega \le b\}$.
%However, Theorem~\ref{thm:R-dominance} ensures
Under general linear constraints, the reduction established in Section V.A relies on the number of vertices in $V$, where $V$ is set of vertices of the preference region (see Theorem 2).
In such case, the number of point location queries performed for each instance is $|V|$.
Since $|V| = O(c^{\lfloor d/2 \rfloor})$, where $c$ is the number of constraints, we can not use the introduced strategies to improve the query time.

\eat{
\begin{mybox}[]{Reviewer 5 - D9}
	Typos expect Fig 7 (c) $\to$ except.
\end{mybox}
}

{\bf D9.} Thanks for careful reviewing.
We checked the entire paper to avoid such errors.
